JWST Validates HST Distance Measurements: Selection of Supernova Subsample Explains Differences in JWST Estimates of Local H0

JWST provides new opportunities to cross-check the HST Cepheid/SNeIa distance ladder, which yields the most precise local measure of H0. We analyze early JWST subsamples (~1/4 of the HST sample) from the SH0ES and CCHP groups, calibrated by a single anchor (N4258). We find HST Cepheid distances agree well (~1 sigma) with all 8 combinations of methods, samples, and telescopes: JWST Cepheids, TRGB, and JAGB by either group, plus HST TRGB and Miras. The comparisons explicitly include the measurement uncertainty of each method in N4258, an oft-neglected but dominant term. Mean differences are ~0.03 mag, far smaller than the 0.18 mag "Hubble tension." Combining all measures produces the strongest constraint yet on the linearity of HST Cepheid distances, 0.994+-0.010, ruling out distance-dependent bias or offset as the source of the tension at ~7 sigma. Yet, measurements of H0 from current JWST subsamples produce large sampling differences whose size and direction we can directly estimate from the full HST set. We show that Delta(H0)~2.5 km/s/Mpc between the CCHP JWST program and the full HST sample is entirely consistent with differences in sample selection. Combining all JWST samples produces a new, distance-limited set of 16 SNeIa at D<25 Mpc and more closely resembles the full sample thanks to "reversion to the mean" of larger samples. Using JWST Cepheids, JAGB, and TRGB, we find 73.4+-2.1, 72.2+-2.2, and 72.1+-2.2 km/s/Mpc, respectively. Explicitly accounting for SNe in common, the combined-sample three-method result from JWST is H0=72.6+-2.0, similar to H0=72.8 expected from HST Cepheids in the same galaxies. The small JWST sample trivially lowers the Hubble tension significance due to small-sample statistics and is not yet competitive with the HST set (42 SNeIa and 4 anchors), which yields 73.2+-0.9. Still, the joint JWST sample provides important crosschecks which the HST data passes.

==> goodruns_mega_R21_10412.2.distapprox.n4258.9.tex <==
\clearpage
\startlongtable
\begin{deluxetable}{lccrrrrrrrrr}
\tabletypesize{\small}
\tablewidth{0pc}
\tablenum{6}
\tablecaption{Approximations for Distance Parameters\label{tb:distpar}}
\tablehead{\colhead{N} & \colhead{Host} & \colhead{SN} & \colhead{$m_{B,i}^0$} & \colhead{$\sigma$} & \colhead{$\mu_{\rm Ceph}^a$} & \colhead{$\sigma$} & \colhead{$M_{B,i}^0$} & \colhead{$\sigma$} & \colhead{$\mu_{\rm host}^b$} & \colhead{$\sigma$} & \colhead{$R^c$} \\
\colhead{} & \colhead{}  & \colhead{} & \multicolumn{7}{c}{(mag)}}
\startdata
N7250 &  31.642  &  0.130  &  2013dy &  12.283  &  0.178  &  -19.357  &  0.222  &  70.0  &  7.5  &  6.7  \\[-0.12cm]
N4536 &  30.870  &  0.061  &  1981B &  11.551  &  0.133  &  -19.320  &  0.147  &  71.2  &  4.9  &  4.6  \\[-0.12cm]
N3972 &  31.644  &  0.096  &  2011by &  12.548  &  0.094  &  -19.103  &  0.136  &  78.7  &  4.9  &  4.6  \\[-0.12cm]
N4424 &  30.854  &  0.133  &  2012cg &  11.487  &  0.192  &  -19.376  &  0.236  &  69.4  &  7.9  &  7.1  \\[-0.12cm]
N4639 &  31.823  &  0.091  &  1990N &  12.454  &  0.124  &  -19.373  &  0.155  &  69.5  &  5.0  &  4.7  \\[-0.12cm]
N4038 &  31.612  &  0.121  &  2007sr &  12.409  &  0.106  &  -19.212  &  0.164  &  74.8  &  5.7  &  5.3  \\[-0.12cm]
M101 &  29.188  &  0.055  &  2011fe &  9.7800  &  0.115  &  -19.421  &  0.127  &  67.9  &  4.0  &  3.7  \\[-0.12cm]
N2442 &  31.459  &  0.073  &  2015F &  12.234  &  0.082  &  -19.230  &  0.111  &  74.2  &  3.7  &  3.6  \\[-0.12cm]
N1365 &  31.378  &  0.061  &  2012fr &  11.900  &  0.092  &  -19.478  &  0.112  &  66.2  &  3.3  &  3.2  \\[-0.12cm]
N5643 &  30.553  &  0.063  &  2013aa &  11.252  &  0.079  &  -19.322  &  0.101  &  71.1  &  3.2  &  3.1  \\[-0.12cm]
N5643 &  30.553  &  0.063  &  2017cbv &  11.208  &  0.074  &  -19.366  &  0.097  &  69.7  &  3.0  &  2.9  \\[-0.12cm]
N5584 &  31.766  &  0.062  &  2007af &  12.804  &  0.079  &  -18.963  &  0.102  &  83.9  &  3.8  &  3.7  \\[-0.12cm]
N1559 &  31.500  &  0.071  &  2005df &  12.141  &  0.086  &  -19.367  &  0.112  &  69.7  &  3.5  &  3.4  \\[-0.12cm]
N5468 &  33.127  &  0.082  &  1999cp &  13.880  &  0.080  &  -19.248  &  0.116  &  73.6  &  3.9  &  3.7  \\[-0.12cm]
N5468 &  33.127  &  0.082  &  2002cr &  13.993  &  0.072  &  -19.135  &  0.111  &  77.5  &  3.9  &  3.7  \\[-0.12cm]
N1448 &  31.298  &  0.051  &  2001el &  12.254  &  0.136  &  -19.046  &  0.146  &  80.8  &  5.5  &  5.1  \\[-0.12cm]
N1448 &  31.298  &  0.051  &  2021pit &  11.752  &  0.200  &  -19.548  &  0.207  &  64.1  &  6.3  &  5.8  \\[-0.12cm]
N5643 &  30.553  &  0.063  &  2013aa &  11.252  &  0.079  &  -19.322  &  0.101  &  71.1  &  3.2  &  3.1  \\[-0.12cm]
N5643 &  30.553  &  0.063  &  2017cbv &  11.208  &  0.074  &  -19.366  &  0.097  &  69.7  &  3.0  &  2.9  \\[-0.12cm]
N2525 &  32.059  &  0.105  &  2018gv &  12.728  &  0.074  &  -19.344  &  0.130  &  70.4  &  4.2  &  4.0  \\[-0.12cm]
N3370 &  32.132  &  0.062  &  1994ae &  12.937  &  0.082  &  -19.196  &  0.104  &  75.4  &  3.5  &  3.4  \\[-0.12cm]
N5861 &  32.232  &  0.105  &  2017erp &  12.945  &  0.107  &  -19.294  &  0.152  &  72.0  &  5.1  &  4.8  \\[-0.12cm]
N3147 &  33.173  &  0.163  &  2021hpr &  13.843  &  0.159  &  -19.358  &  0.230  &  70.0  &  7.7  &  7.0  \\[-0.12cm]
N3147 &  33.173  &  0.163  &  1997bq &  13.821  &  0.141  &  -19.380  &  0.218  &  69.3  &  7.2  &  6.5  \\[-0.12cm]
N3147 &  33.173  &  0.163  &  2008fv &  13.936  &  0.200  &  -19.264  &  0.260  &  73.0  &  9.2  &  8.2  \\[-0.12cm]
M101 &  29.188  &  0.055  &  2011fe &  9.7800  &  0.115  &  -19.421  &  0.127  &  67.9  &  4.0  &  3.7  \\[-0.12cm]
N3021 &  32.473  &  0.162  &  1995al &  13.114  &  0.116  &  -19.368  &  0.203  &  69.6  &  6.7  &  6.1  \\[-0.12cm]
N1309 &  32.552  &  0.069  &  2002fk &  13.209  &  0.082  &  -19.345  &  0.108  &  70.3  &  3.4  &  3.3  \\[-0.12cm]
N3982 &  31.736  &  0.080  &  1998aq &  12.252  &  0.078  &  -19.484  &  0.113  &  66.0  &  3.4  &  3.2  \\[-0.12cm]
N1015 &  32.691  &  0.077  &  2009ig &  13.350  &  0.094  &  -19.346  &  0.123  &  70.3  &  3.9  &  3.7  \\[-0.12cm]
N3447 &  31.947  &  0.049  &  2012ht &  12.736  &  0.089  &  -19.213  &  0.102  &  74.8  &  3.4  &  3.3  \\[-0.12cm]
N5917 &  32.377  &  0.125  &  2005cf &  13.079  &  0.095  &  -19.297  &  0.160  &  72.0  &  5.4  &  5.0  \\[-0.12cm]
U9391 &  32.861  &  0.075  &  2003du &  13.525  &  0.084  &  -19.335  &  0.114  &  70.7  &  3.7  &  3.5  \\[-0.12cm]
N3583 &  32.814  &  0.087  &  ASASSN-15so &  13.509  &  0.093  &  -19.308  &  0.129  &  71.6  &  4.2  &  4.0  \\[-0.12cm]
N2608 &  32.620  &  0.158  &  2001bg &  13.443  &  0.166  &  -19.191  &  0.232  &  75.5  &  8.4  &  7.6  \\[-0.12cm]
N7541 &  32.512  &  0.124  &  1998dh &  13.418  &  0.128  &  -19.095  &  0.181  &  78.9  &  6.7  &  6.2  \\[-0.12cm]
N0691 &  32.838  &  0.114  &  2005W &  13.602  &  0.139  &  -19.250  &  0.182  &  73.5  &  6.3  &  5.8  \\[-0.12cm]
N3254 &  32.343  &  0.084  &  2019np &  13.201  &  0.074  &  -19.141  &  0.114  &  77.3  &  4.0  &  3.8  \\[-0.12cm]
N5728 &  33.101  &  0.208  &  2009Y &  13.514  &  0.115  &  -19.607  &  0.242  &  62.4  &  7.3  &  6.5  \\[-0.12cm]
N7678 &  33.196  &  0.157  &  2002dp &  14.090  &  0.093  &  -19.113  &  0.187  &  78.3  &  6.9  &  6.4  \\[-0.12cm]
M1337 &  33.060  &  0.121  &  2006D &  13.655  &  0.106  &  -19.406  &  0.164  &  68.4  &  5.3  &  4.9  \\[-0.12cm]
N4680 &  32.609  &  0.208  &  1997bp &  13.173  &  0.205  &  -19.440  &  0.296  &  67.3  &  9.8  &  8.5  \\[-0.12cm]
N7329 &  33.252  &  0.122  &  2006bh &  14.030  &  0.079  &  -19.248  &  0.146  &  73.6  &  5.0  &  4.7  \\[-0.12cm]
N0976 &  33.719  &  0.153  &  1999dq &  14.250  &  0.103  &  -19.475  &  0.188  &  66.3  &  5.9  &  5.4  \\[-0.12cm]
N0105 &  34.538  &  0.252  &  2007A &  15.250  &  0.133  &  -19.290  &  0.292  &  72.2  &  10.3  &  9.0  \\[-0.12cm]
\enddata
\tablecomments{(a) Approximate, Cepheid-based distances derived without inclusion of the SNe in each host}
\tablecomments{(b) Cepheid-based distances derived without inclusion of any SNe in any host}
\tablecomments{(c) Empirical host reddening ratio derived from  mass, SFR, using EDA, see section 6.3}
\tablecomments{$m_{B,i}^0$ and error given is an approximation, the simple average from 1 or more SN surveys}
\end{deluxetable}

